BERTtime Stories: Investigating the Role of Synthetic Story Data in Language Pre-training

We describe our contribution to the Strict and Strict-Small tracks of the 2nd iteration of the BabyLM Challenge. The shared task is centered around efficient pre-training given data constraints motivated by human development. In response, we study the effect of synthetic story data in language pre-training using TinyStories: a recently introduced dataset of short stories. Initially, we train GPT-Neo models on subsets of TinyStories, while varying the amount of available data. We find that, even with access to less than 100M words, the models are able to generate high-quality, original completions to a given story, and acquire substantial linguistic knowledge. To measure the effect of synthetic story data, we train LTG-BERT encoder models on a combined dataset of: a subset of TinyStories, story completions generated by GPT-Neo, and a subset of the BabyLM dataset. Our experimentation reveals that synthetic data can occasionally offer modest gains, but overall have a negative influence on linguistic understanding. Our work offers an initial study on synthesizing story data in low resource settings and underscores their potential for augmentation in data-constrained language modeling. We publicly release our models and implementation on our GitHub.

==> tables/table_qualitative_5M_50M.tex <==
\begin{table*}[ht]
    \centering \small
    \begin{tabular}{l|p{15cm}}
    \hline
    \textbf{Model} & \textbf{Generated Text}\\
    \hline
    Prompt & Once there was a small girl named Marie who lived with her mom and dad. Every day, Marie's
        mom and dad would tell her stories. They told her stories about animals, far off lands and even
        her own adventures. One\\
    \hline Original & day, her mom and dad told her a special story: they told her that if she looked under
        the big mineral they had in the garden, she would find a special surprise! Marie was excited to
        look for the surprise. She looked everywhere! She dug holes and searched under rocks and trees.
        But no matter how hard she looked, she could not see any signs of the surprise. Marie was feeling
        sad. But then, one sunny day, she finally found it! Under that big mineral, there was a small
        box. Inside the box was a shiny rock. Marie was so glad to have finally found the surprise. Marie
        was so glad that she showed her mom and dad the surprise. They were just as glad as Marie was
        to see the surprise - it was a special mineral that would protect her from all the bad things
        in the world. Marie keep the mineral near her, so no matter what happened, she would always be
        safe.\\
     \hline
     50M greedy   & would cook yummy food for all his friends. One day, Pandy wanted to make something new. He found
        some spicy carrots and put them in a pot. Then, he started to cook them. He stirred and stirred
        until the carrots were ready to eat. Pandy called his friends over to see the big carrot. They
        all loved it and said, "Yum! Pandy, these are the best!" After eating the spicy carrots, Pandy
        and his friends were very happy. They cooked the big carrot and played in the forest all day long.
        And from that day on, Pandy always made new and yummy treats for his friends.\\
    \hline
     5M greedy   & would go out and work in the forest to make it look better. One day, Pandy was making a big cake
        for his friends. He was very excited. Pandy''s friend, a small bird named Chirpy, saw him cooking
        the cake. Chirpy asked, "What are you cooking, Pandy?" Pandy replied, "I am making a cake for
        my friends. Do you want to help me?" Chirpy looked at the cake and said, "Yes, Pandy! Let''s make
        a cake together!" They put a big bowl on the table and started to cook. But, while they were making
        the cake, it changed. It was bigger than Pandy! Chirpy was surprised and said, "Wow, Pandy! Our
        cake is very big!" Pandy felt embarrassed because he did not forgive Chirpy. They became friends
        and cooked together in the forest all day\\
    \hline
    \end{tabular}
    \caption{Sample generations for \textsc{GPT-Neo} models trained on $\Dtiny[5M]$ and $\Dtiny[50M]$. The prompt and story are included in the training set of both models. We also include the original completion present in the dataset. For a comprehensive qualitative evaluation of all model see Appendix \ref{appendix:tinystories_qualitative}}
    \label{table:greedy_generations_5M_50M}
\end{table*}


